The Devil is in Temporal Token: High Quality Video Reasoning Segmentation

Existing methods for Video Reasoning Segmentation rely heavily on a single special token to represent the object in the keyframe or the entire video, inadequately capturing spatial complexity and inter-frame motion. To overcome these challenges, we propose VRS-HQ, an end-to-end video reasoning segmentation approach that leverages Multimodal Large Language Models (MLLMs) to inject rich spatiotemporal features into hierarchical tokens.Our key innovations include a Temporal Dynamic Aggregation (TDA) and a Token-driven Keyframe Selection (TKS). Specifically, we design frame-level <SEG> and temporal-level <TAK> tokens that utilize MLLM's autoregressive learning to effectively capture both local and global information. Subsequently, we apply a similarity-based weighted fusion and frame selection strategy, then utilize SAM2 to perform keyframe segmentation and propagation. To enhance keyframe localization accuracy, the TKS filters keyframes based on SAM2's occlusion scores during inference. VRS-HQ achieves state-of-the-art performance on ReVOS, surpassing VISA by 5.9%/12.5%/9.1% in J&F scores across the three subsets. These results highlight the strong temporal reasoning and segmentation capabilities of our method. Code and model weights will be released at VRS-HQ.

==> Tables/ReasonSeg_comparison.tex <==
\begin{table}[htbp]
\centering
\caption{Performance comparison with previous methods on ReasonSeg val and test subset. }
\label{ReasonSeg}
\begin{tabular}{l | c c c c}
\toprule[1.2pt]
\multirow{2}{*}{Method} & \multicolumn{2}{c}{ReasonSeg (val)} & \multicolumn{2}{c}{ReasonSeg (test)}  \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}  
& giou & ciou & giou & ciou\\
\midrule
    OVSeg~\cite{liang2023open}   & 28.5 & 18.6 & 26.1 & 20.8 \\
    GRES~\cite{liu2023gres}   & 22.4 & 19.9 & 21.3 & 22.0 \\
    X-Decoder~\cite{zou2023generalized}  & 22.6 & 17.9 &21.7 &16.3\\
    SEEM~\cite{zou2024segment}  & 25.5 & 21.2 & 24.3 & 18.7\\
    Grounded-SAM~\cite{ren2024grounded} &26.0 & 14.5& 21.3 &16.4 \\
    % LISA-7B~\cite{lai2024lisa}  & 44.4 & 46.0 & 36.8 & 34.1 \\
    LISA-7B (ft)~\cite{lai2024lisa}  & 52.9 & 54.0 & 47.3 & 48.4 \\
    % LISA-13B~\cite{lai2024lisa}  & 48.9 & 46.9 & 44.8 & 45.8 \\
    LISA-13B (ft)~\cite{lai2024lisa}  & \underline{56.2} & \underline{62.9} & \underline{51.7} & 51.1 \\
    VISA~\cite{yan2024visa}    & 52.7 & 57.8 & - & - \\
    VideoLISA~\cite{bai2024one}     & \textbf{61.4} & \textbf{67.1} & \textbf{53.8} & \textbf{54.4}\\
    VRS-HQ     & 55.2 & 51.8 & \underline{51.7} & \underline{52.9} \\
\bottomrule[1.2pt]
\end{tabular}
\end{table}

==> Tables/algorithm.tex <==
\begin{algorithm}
\caption{Adaptive Keyframe Selection}
\label{MAKS}
\begin{algorithmic}[1]
\Require $\mathcal{X}_{V}: (T, 3, H, W)$, $\mathcal{X}_{exp}$, $\mathcal{X}_{txt}$
\Ensure $\mathcal{X}_{K}: (3, H, W)$

% clip进行帧采样
\State \textbf{CLIP for global frame sampling}
\State $CLIPScore:(T, 1) \leftarrow CLIP(\mathcal{X}_{V},\mathcal{X}_{exp})$
\State $T_{k} \leftarrow argmax_{i}(CLIPScore[i])$
\State $\mathcal{X}^{f}_{V}:(\hat{T}, 3, H, W),F_{idx}\leftarrow GlobalSample(\mathcal{X}_{V}, T_{k})$

% 计算帧间相似度
\State \textbf{Calculate the token similarity}
\State $h_{seg}, h_{tak} \leftarrow MLP(MLLM(\mathcal{X}^{f}_{V}, \mathcal{X}_{txt}))$
\State $S_{1}: (\hat{T}, 1) \leftarrow Softmax(CosSim(h_{seg}, h_{tak}))$
\State $h'_{tak} \leftarrow TDA(h_{seg}, h_{tak}, S_{1})$

% 将各帧分别作为关键帧并送入SAM2模型中得到object score
\State \textbf{Generate the Object score}
\For {$i=0 \to \hat{T}$}
\State  $S^{i}_{2} \leftarrow SAM2(\mathcal{X}^{f}_{V}[i], h'_{tak})$
\EndFor
\State $S'_{2} : (\hat{T}, 1) \leftarrow Softmax(S_{2})$

% 将三种分数相结合来定位关键帧
\State \textbf{Locate the Keyframe}
\State $TotalScore : (\hat{T}, 1) \leftarrow S_{1} + S'_{2}$
\State $\mathcal{X}_{K} : (3, H, W) \leftarrow \mathcal{X}^{f}_{V}[argmax_{i}(TotalScore[i])]$
\end{algorithmic}
\end{algorithm}

==> Tables/training_frame_ablation.tex <==
\begin{table}[htbp]
\centering
\caption{Ablation study of the number of the frames for training. }
\label{frame number ablation}
\scalebox{0.95}{
\begin{tabular}{c | c c c c c c}
\toprule[1.2pt]
\multirow{2}{*}{Num. of Frames} & \multicolumn{3}{c}{referring} & \multicolumn{3}{c}{reasoning} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& $\mathcal{J}$ & $\mathcal{F}$ & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & $\mathcal{J}\&\mathcal{F}$ \\
\midrule
    1       & & & & & & \\
    2     & & & & & &\\  % 之后也可以去掉不放
    3    & & & & & &\\
    5     & & & & & &\\
\bottomrule[1.2pt]
\end{tabular}
}
\end{table}

==> sec/3_task_defination.tex <==
\section{Task Defination}
The task of Video Reasoning Segmentation can be briefly outlined as follows.
Given a video clip consisting of $T$ frames $\mathcal{X}_{V}\in{\mathbb{R}^{T\times{3}\times{H}\times{W}}}$, where $H$ and $W$ denote the height and width of each frame respectively, along with a high-level textual instruction $\mathcal{X}_{txt}$ incorporating human intent and world knowledge,
VRS aims to design a model $\mathcal{M}$ to interpret and translate $\mathcal{X}_{txt}$ into the binary segmentation mask sequence $\mathcal{X}_{M}\in{\mathbb{R}^{T\times{H}\times{W}}}$ for each frame. 
The formulation of the specific process is as follows:
\begin{equation}
\mathcal{X}_{M}=\mathcal{M}(\mathcal{X}_{V}, \mathcal{X}_{txt})
\end{equation}

% In contrast to Ref-VOS tasks providing explicit descriptions, such as "the person skateboarding," ReasonVOS typically employs expressions that integrate common-sense knowledge, such as "tool(s) for holding garbage" or temporal logic like "the ship(s) moving from left to right at the highest speed." This raises higher demands on the model's capabilities of temporal relationship comprehension and complex scenario reasoning.
% equipping MLLMs with advanced environmental interactions and real-world comprehension capabilities.
% our approach aims to utilize both inputs to identify and locate the target within the video, generating a binary mask sequence for each frame. 
